Universal approximation of flows of control systems by recurrent neural networks

We consider the problem of approximating flow functions of continuous-time dynamical systems with inputs. It is well-known that continuous-time recurrent neural networks are universal approximators of this type of system. In this paper, we prove that an architecture based on discrete-time recurrent neural networks universally approximates flows of continuous-time dynamical systems with inputs. The required assumptions are shown to hold for systems whose dynamics are well-behaved ordinary differential equations and with practically relevant classes of input signals. This enables the use of off-the-shelf solutions for learning such flow functions in continuous-time from sampled trajectory data.

==> 99-prelim-old.tex <==
\subsection{Notation}
The indicator function of a set $A$ is written $\Indic_{A}$,
and the identity function on $A$ is written $\Id_A: A \to A$.
Vectors $v \in \Reals^{d}$ are written $v = (v_1, \dots, v_d)$.
Sequences are written $(z_k)_{k=0}^{\infty}$, or by the short-hand $(z_k)$.
The space of sequences with values in a set $A$ is written
${\SeqSp{A} := \Set{(z_k)_{k=0}^{\infty}: z_k \in A}}$.
The space of continuous functions $f : A \to \Reals^n$ on a compact set
$A \subset \Reals^m$ is written $C_n(A)$.
For a set $A \subset \Reals^n$ and $\eps > 0$, $N_\eps(A)$ denotes the (closed) $\eps$-neighbourhood of $A$,
i.e., the set of points at most $\eps$ distance away from $A$.
If $A$ is compact, then so is $N_\eps(A)$.

\subsection{Flows of controls systems in continuous-time}\label{ssec:flows-defn}
In this paper we consider finite-dimensional
time-invariant control systems in continuous-time with state evolving in
an open set $\States \subset \Sp{x}$.
Such systems can be described abstractly by a \textit{flow function}
\begin{equation}
    {\Flow: \Reals_{\geq 0} \times \States \times \Controls \to \States}
\end{equation}
where $\Controls$ is a given set of (control) inputs
$u: \Reals_{\geq 0}\to \Reals^{d_u}$.
The flow satisfies the following properties (cf.~Sontag~\cite[Chapter~2]{Sontag98}):
\begin{itemize}
    \item Identity: $\Flow(0, x, u) = x$
    \item Semigroup: $\Flow(s + t, x, u) = \Flow(t, \Flow(s, x, u), u^s)$
\end{itemize}
for all $x \in X$, $u \in \Controls$ and $s, t \geq 0$.
Here $u^s \in \Controls$ denotes the input $u$ shifted by $s > 0$ time units, i.e.,
$u^s(t) := u(t + s)$.
The function $\xi(t) := \Flow(t, x, u)$ for $t \geq 0$ is the trajectory of the system
with initial state $x$ when the applied control is $u$.

\subsection{Neural networks}
In this paper, a \emph{(feedforward) neural network} is any function $f: \Reals^{m} \to \Reals^n$
which can be written as \Cmt{Simplify this}
\begin{equation}\label{eq:ff-network}
    h = a_2 \circ \sigma_p \circ a_1
\end{equation}
where ${\sigma_p: \Reals^p \to \Reals^p}$ is the diagonal mapping such that the \emph{activation function} $\sigma: \Reals \to \Reals$
is applied to each coordinate, i.e.,
${\sigma_p(v) = (\sigma(v_1), \dots, \sigma(v_p))}$ 
for $v \in \Reals^p$.
and ${a_1: \Reals^m \to \Reals^p}$
and ${a_2: \Reals^p \to \Reals^n}$ are affine.
In other words, $h$ may be written as
\begin{equation*}
    h(x) = C \sigma_p(Ax + b) + d
\end{equation*}
for $A \in \Reals^{p \times m}$, $b \in \Reals^p$,
$C \in \Reals^{n \times p}$, $d \in \Reals^{n}$.
In practical applications these are usually known as networks with
\emph{one hidden layer}.
We let $\Nets^{m, n}_{\sigma, p}$ be the class of such networks and define
\begin{equation*}
    \Nets^{m, n}_{\sigma} :=
    \bigcup_{p = 1}^{\infty} \Nets^{m,n}_{\sigma, p}.
\end{equation*}
Hornik~\cite{Hornik91} has shown that networks in $\Nets^{n, m}_{\sigma}$
are~\textit{universal approximators} in the following sense:
\begin{theorem}[Hornik~\cite{Hornik91}]\label{thm:ua-ffnet}
    Let $\sigma : \Reals \to \Reals$ be bounded, continuous and nonconstant.
    For any compact set $X \subset \Reals^m$, $\Nets^{n, m}_\sigma$ is dense in $C_n(X)$.
    In other words, for any function $f: X \to \Reals^n$ and $\eps > 0$ there is a network
    $h \in \Nets^{n, m}_{\sigma}$ such that
    \begin{equation*}
        \sup_{x \in X}\Norm{f(x) - h(x)} < \eps.
    \end{equation*}
\end{theorem}
Throughout the paper, we shall denote by ${\sigma: \Reals \to \Reals}$ a function satisfying
the assumptions of Theorem~\ref{thm:ua-ffnet}.
\Cmt{Expand on Theorem 1 a bit more; why it is important for this paper.}

\subsection{Discrete-time systems and recurrent neural networks}

We shall need to consider discrete-time systems given by state-space models
of the form
\begin{equation}\label{eq:dt-sys}
    x_{k+1} = f(x_k, u_k), \ k \in \PInts,
\end{equation}
where $x_k \in \Sp{x}$ is the {state} of the system and $u_k \in \Sp{u}$
is the input value at timestep $k$.
Informally, we will refer to $f$ as the `right-hand side' of the system.
For such a system, we define the (discrete-time) flow
$\dflow_{f}: \PInts \times \Sp{x} \times \SeqSp{\Sp{u}} \to \Sp{x}$ as
\begin{equation*}
   \dflow_f(n, x, u) := x_n,
\end{equation*}
where $x_n$ is the $n$-th element of the state sequence generated by the recursion~\eqref{eq:dt-sys},
with the initial state $x_0 = x$ and input sequence $u = (u_k)_{k=0}^{\infty}$.
Equivalently, we can define $\dflow_f$ by the following recursion:
\begin{equation*}
\begin{aligned}
    \dflow_f(0, x, u) &= x, \\
    \dflow_f(n + 1, x, u) &= f(\dflow_f(n, x, u), u_n).
\end{aligned}
\end{equation*}

\Cmt{Starting from II.C till this point, \st{Definition 2} can be moved directly after II.A under a new subsection \emph{Discrete-time dynamical systems and their flows}. Then we continue with a new subsection \emph{Neural Networks: Feedforward and Recurrent}. Here, we can start with FFN and continue to RNN.}

\Cmt{Is Definition 2 really required? Can we not be explicit when we state Theorem 3?}

\Cmt{"We denote by $\Nets^{0}_{\sigma}$ the class of networks" essentially makes it natural to bring RNN directly after FNN}

We denote by $\Nets^{0}_{\sigma}$ the class of networks such that
the affine function at the output of the network
(i.e., $a_2$ in equation~\eqref{eq:ff-network}) is the identity.
A recurrent neural network is then simply a discrete-time dynamical
system for which the right hand side is a network in $\Nets^0_{\sigma}$:
\begin{definition}[Recurrent neural network]
A \emph{recurrent neural network} is a dynamical system of the form
\begin{equation*}
    z_{k + 1} = \sigma_{d_z}(A z_k + B u_{k} + b).
\end{equation*}
where $z \in \Sp{z}$, $u \in \Sp{u}$.

    \Cmt{
     A \emph{recurrent neural network} is a discrete-time dynamical system of the form $ z_{k + 1} = h(z_k), z_k \in \Reals^{d_z},$ where, the right-hand side, $h(\cdot)$, is a feedforward neural network defined according to...
     Moreover, we denote such a specific class of feedforward neural network as $\Nets^0_{\sigma}$.\\
     Remark: The class of neural network $\Nets^0_{\sigma}$ coincides with \eqref{eq:ff-network} where the affine function $a_2$ is the identity.\\
     \emph{You get the idea I hope. Change the specifics accordingly.}
     }
\end{definition}

Finally, we adapt the following definition from Sontag~\cite{Sontag92},
which provides a notion of approximating a discrete-time dynamical system
by a second system.
\begin{definition}\label{def:simulation}
    Consider two dynamical systems
    \begin{equation*}
        \begin{aligned}
            x_{k + 1} &= f(x_k, u_k), \\
            z_{k + 1} &= g(z_k, u_k).
        \end{aligned}
    \end{equation*}
    
    Given $\eps > 0$, $N \in \PInts$ and sets ${K_x \subset \Sp{x}}$, ${K_u \subset \Sp{u}}$,
    we say that \emph{$\dflow_g$ simulates $\dflow_f$ on $K_x, \ K_u$ up to time $N$ and up to accuracy $\eps$} 
    if there exist continuous mappings $\gamma: \Sp{z} \to \Sp{x}$ and $\beta: \Sp{x} \to \Sp{z}$ such that
    for any $x \in K_x$ and $u \in \SeqSp{K_u}$ we have
    \begin{equation}\label{eq:sim}
        \Norm{\dflow_f(n, x, u) - \gamma(\dflow_g(n, \beta(x), u))} < \eps, \ n = 0, \dots, N.
    \end{equation}
\end{definition}
